A search for transits among the {\delta} Scuti variables in Kepler

We search for transits around all known pulsating {\delta} Sct variables (6500 K < Teff < 10 000 K) in the long-cadence Kepler data after subtracting the pulsation signal through an automated routine. To achieve this, we devise a simple and computationally inexpensive method for distinguishing between low-frequency pulsations and transits in light curves. We find 3 new candidate transit events that were previously hidden behind the pulsations, but caution that they are likely to be false positive events. We also examined the Kepler Objects of Interest catalog and identify 13 additional host stars which show {\delta} Sct pulsations. For each star in our sample, we use the non-detection of pulsation timing variations for a planet that is known to be transiting a {\delta} Sct variable to obtain both an upper limit on the mass of the planet and the expected radial velocity semi-amplitude of the host star. Simple injection tests of our pipeline imply 100% recovery for planets of 0.5 RJup or greater. Extrapolating our number of Kepler {\delta} Sct stars, we expect 12 detectable planets above 0.5 RJup in TESS. Our sample contains some of the hottest known transiting planets around evolved stars, and is the first complete sample of transits around {\delta} Sct variables. We make available our code and pulsation-subtracted light curves to facilitate further analysis.

==> figures/flowchart_gen.tex <==
% \tikzstyle{startstop} = [rectangle, rounded corners, minimum width=3cm, minimum height=1cm,text centered, draw=black, fill=red!30]
% \tikzstyle{io} = [trapezium, trapezium left angle=70, trapezium right angle=110, text width=0.2*\columnwidth, 
%   anchor=west,
%   minimum height=1cm,draw=black, fill=blue!30]
% \tikzstyle{process} = [rectangle, minimum width=3cm, minimum height=1cm, text centered, text width=3cm, draw=black, fill=orange!30]
% \tikzstyle{decision} = [rectangle, minimum width=3cm, minimum height=1cm, text centered, text width=3cm, draw=black, fill=green!30]
% \tikzstyle{arrow} = [thick,->,>=stealth]

\newcommand{\transreceptor}[3]{%
  \path [linepart] (#1.east) -- node [above] {\scriptsize #2} (#3);}
  
\begin{figure}
    \centering
    
    \begin{tikzpicture}[
        node distance = 10mm and 10mm,
        start chain = A going below,
        base/.style = {draw, rounded corners, align=center, minimum width=3cm, minimum height=1cm, text centered, text width=3cm,  on chain=A,drop shadow},
        startstop/.style = {base, rectangle, rounded corners, fill=red!20},
        process/.style = {base, rectangle, fill=blue!15},
        io/.style = {base, rectangle, rounded corners, 
                         %trapezium left angle=70, trapezium right angle=110,
                         fill=blue!20},
        decision/.style = {base, rectangle, fill=green!75!black!25},
        back group/.style={fill=yellow!20,rounded corners, draw=black!50, dashed, inner xsep=15pt, inner ysep=10pt},
        arrow/.style = {->,>=stealth},
        every edge quotes/.style = {auto=right}]
                    ]

    \node [startstop]       {Input light curve files};            % 1
    \node [process, yshift=-0.3cm]       {Spline fit \& sigma clip each quarter};            % 2
    \node [process]       {Stitch light curve};            % 3
    \node [process]         {Calculate amplitude spectrum}; % 4
    \node [process]              {Estimate $f$, $a$, $\phi$ of maximum amplitude signal}; %5
    \node [decision]        {Is $a$ above 5~SNR?}; %6
    \node [startstop]         {Output cleaned light curve}; %7
    \node [io]         {TLS search};             % 8
    \node [decision,                             % 9
      right=of A-6]    {Is signal transit or intrinsic?};
    \node [process,                             % 10
      above=of A-9]    {Fit signal using initial estimate of parameters};
    \node [process,                             % 11
      right=of A-4, above=of A-10]    {Subtract signal from light curve};
    \node [process, right=of A-8]         {BLS search};             % 12
    \node [process, below=of A-8]         {Manual inspection};             % 13
    \coordinate [below=of A-7, yshift=0.5cm] (d1);
    
    \begin{scope}[on background layer]
        \node (bk1) [back group] [fit=(A-2) (A-3)]{};
        \node (bk2) [back group] [fit=(A-4) (A-5) (A-9) (A-10) (A-11)]{};
        \node (bk3) [back group] [fit=(A-8) (A-12) (A-13)]{};
        % \node [draw, thick, green!50!black, fill=green!75!black!25, rounded corners, fit=(p-1), inner xsep=15pt, inner ysep=10pt] {};
    \end{scope}
    
    \draw [arrows=-Stealth] 
        (A-1) edge[]          (A-2)
        (A-2) edge[]    (A-3)
        (A-3) edge[]       (A-4)
        (A-4) edge[]            (A-5)
        (A-5) edge[]          (A-6)
        (A-6) edge["N"]          (A-7)       % <-- by ' is swapped label position
        % (A-9.south) edge[] (A-7.east)
        (A-11) edge[]       (A-4)
        (A-6) edge["Y"]       (A-9)
        (A-9) edge["Intrinsic"]       (A-10)
        (A-10) edge[]       (A-11)
        (A-7) edge[]       (A-8)
        % (A-8) [stealth-stealth]      (A-12)
        % (A-9) |- (A-7.east)
        (A-8) edge[] (A-13)
        
        % (d1) -| (A-12)
        (A-12.south) |- (A-13)
        % (A-7.south) |- (A-12)
        ;
    

    \draw [arrow] (d1) -| (A-12);
    \draw [arrow] (A-9) |- node[anchor=south,xshift=0.6cm] {Transit} (A-7.east);
    
    % \node [below=of A-9, xshift=0.6cm, yshift=0.6cm] {Transit};
    
    \node [above=of A-2, xshift=1.1cm, yshift=-0.6cm] {\textit{Preprocessing}};
    \node [above=of A-11, xshift=1cm, yshift=-0.6cm] {\textit{Cleaning}};
    \node [above=of A-12, xshift=1cm, yshift=-0.6cm] {\textit{Transit search}};
    
    
    \end{tikzpicture}

    \caption{Flowchart of the main functions of the pipeline.}
    \label{fig:pipeline}
\end{figure}

==> tables/injection_dist.tex <==
\begin{table}
    \centering
    \begin{tabular}{ll}
    \hline
    Parameter   &   Distribution \\
    \hline  
    \hline
    \end{tabular}
    \caption{Distributions used in the injection testing.}
    \label{tab:inj_dist}
\end{table}
